Enwar 3.0: An Agentic Multi-Modal LLM Orchestrator for Situation-Aware Beamforming, Blockage Prediction, and Handover Management

Maintaining robust millimeter-wave (mmWave) connectivity in vehicular networks requires real-time adaptation to environmental dynamics, sensor degradation, and link variability. This paper presents Enwar 3.0, an environment-aware reasoning framework that unifies multi-modal sensing, agentic large language models (LLMs), and context-driven model selection for predictive beamforming, blockage detection, and handover management. Building upon prior iterations of Enwar, the proposed architecture integrates a classifier-driven assessment of sensor health with a primed LLM that orchestrates multiple specialized agents through structured, task-aware prompting. A novel synthetic degradation pipeline enables the training of a sensor degradation classifier that detects real-time impairments across camera, radar, LiDAR, and GPS inputs, achieving over 99% accuracy. The LLM, trained via chain-of-thought (CoT) priming and human-in-the-loop feedback, coordinates agent calls for beam selection, blockage forecasting, and environment perception while dynamically loading sensor-specific models based on environmental context. Extensive evaluations across 15 sensor combinations demonstrate that Enwar 3.0 delivers state-of-the-art performance in both predictive accuracy and interpretability, with beam selection accuracy exceeding 88%, blockage F1-scores surpassing 98%, and reasoning correctness reaching 87% on complex decision prompts. This work establishes a scalable foundation for LLM-integrated wireless systems that reason, perceive, and adapt in real-time.

==> Acronym.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

% \acrodef{}[]{}
\acrodef{XAI}[XAI]{explainable AI}
\acrodef{QA}[Q\&A]{question-answer}
\acrodef{PPO}[PPO]{proximal policy optimization}
\acrodef{DRL}[DRL]{deep reinforcement learning}
\acrodef{RL}[RL]{reinforcement learning}
\acrodef{TransFusion}[TransFusion]{transformer-fusion}
\acrodef{RLHF}[RLHF]{reinforcement learning from human feedback}
\acrodef{AUC-ROC}[AUC-ROC]{area under the receiver operating characteristic curve}
\acrodef{BEV}[BEV]{bird's-eye view}
\acrodef{CoT}[CoT]{chain-of-thought}
\acrodef{KB}[KB]{knowledge base}
\acrodef{PEFT}[PEFT]{parameter efficient fine-tuning}
\acrodef{DBA}[DBA]{distance-based accuracy}
\acrodef{APL}[APL]{actual power loss}
\acrodef{ULA}[ULA]{uniform linear array}
\acrodef{RSU}[RSU]{roadside unit}
\acrodef{DoP}[DoP]{dilution of precision}
\acrodef{FAISS}[FAISS]{Facebook AI Similarity Search}
\acrodef{YOLO}[YOLO]{You Only Look Once}
\acrodef{LSTM}[LSTM]{long short-term memory}
\acrodef{CNN}[CNN]{convolutional neural network}
\acrodef{RANSAC}[RANSAC]{random sample consensus}
\acrodef{DBSCAN}[DBSCAN]{density-based spatial clustering of applications with noise}
\acrodef{LLM}[LLM]{large language model}
%\acrodef{LMM}[LMM]{large multi-modal model}
\acrodef{MLLM}[MLLM]{multi-modal large language model}
\acrodef{RAG}[RAG]{retrieval-augmented generation}
\acrodef{ISAC}[ISAC]{integrated sensing and communication}
\acrodef{ZSM}[ZSM]{zero-touch network and service management}
\acrodef{DT}[DT]{digital twin}
\acrodef{I2T}[I2T]{image-to-text}
\acrodef{I2V}[I2V]{infrastructure-to-vehicle}
\acrodef{GTE}[GTE]{general text embeddings}
\acrodef{GLUE}[GLUE]{General Language Understanding Evaluation}
\acrodef{MMLU}[MMLU]{Massive Multitask Language Understanding}


%%%%%%%%%%%%%%%%%%%%%%% Predefined
\acrodef{IoT}[IoT]{Internet of things}
\acrodef{PDCP}[PDCP]{packet data convergence protocol}
\acrodef{RATs}[RATs]{radio access technologies}
% \acrodefplural{RAT}[RAT]{radio access technologies}
\acrodef{AP}[AP]{access point}
\acrodef{BS}[BS]{base station}
\acrodef{MP-TCP}[MP-TCP]{Multipath transmission control protocol}
\acrodef{5QI}[5QI]{\ac{5G} \ac{QoS} identifier}
\acrodef{NSI}[NSI]{network slice instance}
\acrodef{ATSSS}[ATSSS]{access traffic steering, switching and splitting}
\acrodef{CA}[CA]{coordination area}
\acrodef{TRP}[TRP]{transmission-reception point}
\acrodef{SON}[SON]{self-organizing network}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{eMBB}[eMBB]{enhanced mobile broadband}
\acrodef{mMTC}[mMTC]{massive machine type communication}
\acrodef{uRLLC}[uRLLC]{ultra-reliable low latency communication}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{LTE}[LTE]{Long Term Evolution}
\acrodef{LTE-A}[LTE-A]{LTE-Advanced}
\acrodef{3GPP}[3GPP]{3rd Generation Partnership Project}
\acrodef{FFR}[FFR]{fractional frequency reuse}
\acrodef{SFR}[SFR]{soft frequency reuse}
\acrodef{ICI}[ICI]{inter-cell interference}
\acrodef{ICIC}[ICIC]{inter-cell interference coordination}
\acrodef{eICIC}[eICIC]{enhanced \ac{ICIC}}
\acrodef{ABS}[ABS]{absolute blank subframe}
\acrodef{TP}[TP]{transmission point}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{eNB}[eNB]{eNodeB}
\acrodef{RAN}[RAN]{radio access network}
\acrodef{C-RAN}[C-RAN]{cloud-RAN}
\acrodef{RRH}[RRH]{remote radio head}
\acrodef{BBU}[BBU]{baseband unit}
\acrodef{CS}[CS]{coordinated scheduling}
\acrodef{CB}[CB]{coordinated beamforming}
\acrodef{JT}[JT]{joint transmission}
\acrodef{NC-JT}[NC-JT]{non-coherent \ac{JT}}
\acrodef{C-JT}[C-JT]{coherent \ac{JT}}
\acrodef{DPS}[DPS]{dynamic point selection}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{UE}[UE]{user equipment}
\acrodef{RNTP}[RNTP]{relative narrowband transmission power}
\acrodef{eRNTP}[eRNTP]{enhanced \ac{RNTP}}
\acrodef{OI}[OI]{overload indicator}
\acrodef{HII}[HII]{high interference indicator}
\acrodef{HG}[HG]{Hermite-Gaussian}
\acrodef{CQI}[CQI]{channel quality indicator}
\acrodef{PMI}[PMI]{precoding matrix indicator}
\acrodef{RI}[RI]{rank indicator}
\acrodef{HetNet}[HetNet]{heterogeneous network}
\acrodef{mmWave}[mmWave]{millimeter wave}
\acrodef{SINR}[SINR]{signal-to-interference-plus-noise ratio}
\acrodef{SC}[SC]{single-carrier}
\acrodef{SM-OFDM}[SM-OFDM]{Spatial modulation-OFDM}
\acrodef{GB}[GB]{guard band}
\acrodef{DL}[DL]{downlink}
\acrodef{UL}[UL]{uplink}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{GBR}[GBR]{guaranteed bit-rate}
\acrodef{GFDM}[GFDM]{generalized orthogonal frequency division multiplexing}
\acrodef{RSRP}[RSRP]{reference signal received power}
\acrodef{CSI-RSRP}[CSI-RSRP]{CSI-reference signal received power}
\acrodef{5G}[5G]{fifth generation}
\acrodef{4G}[4G]{fourth generation}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{SISO}[SISO]{single-input single-output}
\acrodef{GCoMP}[GCoMP]{generalized CoMP}
\acrodef{CU}[CU]{central unit}
\acrodef{DU}[DU]{distributed unit}
\acrodef{RU}[RU]{remote unit}
\acrodef{FH}[FH]{fronthaul}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{NLoS}[NLoS]{non-line-of-sight}
\acrodef{TBS}[TBS]{terrestrial base station}
\acrodef{IoE}[IoE]{Internet of Everything}
\acrodef{SI}[SI]{self-interference}
\acrodef{FBS}[FBS]{flying base station}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PRB}[PRB]{physical resource block}
\acrodef{PSK}[PSK]{phase-shift keying}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{ostbc}[OSTBC]{orthogonal space time block codes}
\acrodef{OOBE}[OOBE]{out-of-band emission}
\acrodef{svd}[SVD]{singular value decomposition}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QoS}[QoS]{quality-of-service}
\acrodef{ITS}[ITS]{intelligent transportation system}
% \acrodef{TRxP}[TRxP]{transmission reception point}
\acrodef{HO}[HO]{handover}
\acrodef{TUBITAK}[TUBITAK]{Scientific and Technological Research Council of Turkey}
\acrodef{MBB}[MBB]{\textit{Make-Before-Break}}
\acrodef{RACH}[RACH]{\textit{Random Access Channel}}
\acrodef{eMTC}[eMTC]{\textit{enhanced machine type communication}}
\acrodefplural{GBR}[GBR]{guaranteed bit rate}
\acrodef{RB}[RB]{resource block}
\acrodef{PPP}[PPP]{Poisson point process}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{RSSI}[RSSI]{received signal strength indicator}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{CFR}[CFR]{channel frequency response}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{ISI}[ISI]{inter-symbol interference}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{ISD}[ISD]{inter-site distance}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{BER}[BER]{bit error rate}
\acrodef{CSF}[CSF]{channel shortening filter}
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{TDD}[TDD]{time-division duplex}
\acrodef{FDD}[FDD]{frequency-division duplex}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{MSSNR}[MSSNR]{maximum shortening signal-to-noise ratio}
\acrodef{PSD}[PSD]{power spectral density}
\acrodef{QPSK}[QPSK]{Quadrature Phase Shift Keying}
\acrodef{MMSE}[MMSE]{ minimum mean-squared error}
\acrodef{Rx}[Rx]{receiver}
\acrodef{Tx}[Tx]{transmitter}
\acrodef{TRCPR}[TRCPR]{\ac{Tx}-\ac{Rx} channel-based phase rotation}
\acrodef{TOCPR}[TOCPR]{\ac{Tx}-only channel-based phase rotation}
\acrodef{ML}[ML]{maximum likelihood}
\acrodef{SDCO}[SDCO]{spatially Distributed constellation obfuscation}
\acrodef{PDF}[PDF]{probability density function}
\acrodef{SER}[SER]{symbol error rate}
\acrodef{MISO}[MISO]{multiple-input single-output}
\acrodef{FD}[FD]{full-duplex}
\acrodef{AN}[AN]{artificial noise}
\acrodef{SC}[SC]{secrecy capacity}
\acrodef{IBFD}[IBFD]{in-band full-duplex}
\acrodef{KPI}[KPI]{key performance indicator}
\acrodef{VR}[VR]{virtual reality}
\acrodef{AR}[AR]{augmented reality}
\acrodef{6G}[6G]{sixth generation}
\acrodef{RF}[RF]{radio frequency}
\acrodef{PZ}[PZ]{protected zone}
\acrodef{SIC}[SIC]{\ac{SI} cancellation}
\acrodef{SA}[SA]{simulated annealing }
\acrodef{AI}[AI]{artificial intelligence}
\acrodef{BCD}[BCD]{block coordinate descent}
\acrodef{EE}[EE]{energy efficiency}


==> tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% DRL Performance Table %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[h]
\centering
\caption{Comparison of DRL Agent vs. Baselines in Agent Selection Task}
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{Avg. Reward} & \textbf{\% Optimal Actions} & \textbf{\% Degraded Sensors Used} \\
\hline
Random Policy    & 0.69 & 13.2\% & 61.5\% \\
Rule-Based Policy & 1.14 & 67.1\% & 38.7\% \\
\textbf{\ac{PPO} Agent (Proposed)}  & \textbf{1.45} & \textbf{86.6\%} & \textbf{12.9\%} \\
\hline
\end{tabular}
\label{tab:agent_selection_comparison}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Agent Performance Table %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}
\caption{Agent Performance for $t+1$ with $[M=16, Q=64]$}
\label{tab: agent_performance}
\centering
\begin{tabular}{|c|c|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Modality}} & \multirow{2}{*}{\textbf{Preprocessing}} & \multicolumn{3}{c|}{\textbf{Beam Prediction}} & \multicolumn{3}{c|}{\textbf{Blockage Prediction}} \\ \cline{3-8} 
 & \textbf{Time (ms)} & \multicolumn{1}{c|}{\textbf{APL}} & \multicolumn{1}{c|}{\textbf{Accuracy}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inference \\ Time (ms)\end{tabular}} & \multicolumn{1}{c|}{\textbf{F1 Score}} & \multicolumn{1}{c|}{\textbf{AUC-ROC}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inference \\ Time (ms)\end{tabular}} \\ \hline
 
camera\_gps\_lidar & 43.3 & \multicolumn{1}{c|}{-0.009220} & \multicolumn{1}{c|}{88.5\%} &  187.7 & \multicolumn{1}{c|}{91.2\%} & \multicolumn{1}{c|}{0.897} & 127.5 \\ \hline

camera\_radar\_lidar & 54.3 & \multicolumn{1}{c|}{-0.009314} & \multicolumn{1}{c|}{88.3\%} & 199.6 & \multicolumn{1}{c|}{94.0\%} & \multicolumn{1}{c|}{0.928} & 128.9 \\ \hline
 
camera\_gps\_radar\_lidar & 56.0 & \multicolumn{1}{c|}{-0.009660} & \multicolumn{1}{c|}{85.8\%} & 206.7 & \multicolumn{1}{c|}{93.1\%} & \multicolumn{1}{c|}{0.914} & 137.2 \\ \hline
 
camera\_lidar & 42.4 & \multicolumn{1}{c|}{-0.009668} & \multicolumn{1}{c|}{85.6\%} & 185.8 &  \multicolumn{1}{c|}{96.2\%} & \multicolumn{1}{c|}{0.955} & 121.8 \\ \hline
 
camera\_gps\_radar & 18.3 & \multicolumn{1}{c|}{-0.01469} & \multicolumn{1}{c|}{84.9\%} & 183.3 & \multicolumn{1}{c|}{92.3\%} & \multicolumn{1}{c|}{0.911} & 121.2 \\ \hline
 
camera\_radar & 17.8 & \multicolumn{1}{c|}{-0.02125} & \multicolumn{1}{c|}{84.2\%} & 159.5 & \multicolumn{1}{c|}{98.4\%} & \multicolumn{1}{c|}{0.988} & 95.7 \\ \hline
 
camera\_gps & 4.96 & \multicolumn{1}{c|}{-0.02844} & \multicolumn{1}{c|}{83.7\%} & 149.3 & \multicolumn{1}{c|}{94.4\%} & \multicolumn{1}{c|}{0.931} & 109.4 \\ \hline
 
gps\_lidar\_radar & 51.8 & \multicolumn{1}{c|}{-0.03553} & \multicolumn{1}{c|}{83.0\%} & 174.3 & \multicolumn{1}{c|}{89.9\%} & \multicolumn{1}{c|}{0.889} & 125.0 \\ \hline
 
camera\_only & 4.11 & \multicolumn{1}{c|}{-0.03705} & \multicolumn{1}{c|}{82.8\%} & 122.6 & \multicolumn{1}{c|}{98.1\%} & \multicolumn{1}{c|}{0.983} & 89.8 \\ \hline
 
gps\_radar & 13.5 & \multicolumn{1}{c|}{-0.03979} & \multicolumn{1}{c|}{81.9\%} & 131.7 & \multicolumn{1}{c|}{89.3\%} & \multicolumn{1}{c|}{0.880} & 96.1 \\ \hline
 
gps\_lidar & 38.4 & \multicolumn{1}{c|}{-0.08013} & \multicolumn{1}{c|}{76.6\%} & 141.0 & \multicolumn{1}{c|}{84.1\%} & \multicolumn{1}{c|}{0.855} & 121.6 \\ \hline
 
radar\_lidar & 50.7 & \multicolumn{1}{c|}{-0.1427} & \multicolumn{1}{c|}{74.4\%} & 158.2 & \multicolumn{1}{c|}{91.8\%} & \multicolumn{1}{c|}{0.902} & 124.1 \\ \hline
 
radar\_only & 12.4 & \multicolumn{1}{c|}{-0.1602} & \multicolumn{1}{c|}{72.4\%} & 126.5
& \multicolumn{1}{c|}{93.7\%} & \multicolumn{1}{c|}{0.922} & 92.6 \\ \hline
 
lidar\_only & 37.9 & \multicolumn{1}{c|}{-0.1743} & \multicolumn{1}{c|}{65.7\%} & 130.7 & \multicolumn{1}{c|}{87.9\%} & \multicolumn{1}{c|}{0.872} & 117.3 \\ \hline
 
gps\_only & $<1$ & \multicolumn{1}{c|}{-0.2151} & \multicolumn{1}{c|}{59.0\%} & 87.4 & \multicolumn{1}{c|}{61.7\%} & \multicolumn{1}{c|}{0.603} & 37.3 \\ \hline
\end{tabular}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Handover Strategies Table %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h]
\centering
\caption{Comparison of Handover Strategies, $k = 5$}
\label{tab:handover_eval}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Metric} & \textbf{No} & \textbf{Immediate} & \textbf{Oracle} & \textbf{\textsc{Enwar 3.0}} \\
& \textbf{Handover} & & & \\
\hline
APL @ $t + k$ & -5.10 & +0.71 & \textbf{+2.53} & +1.82 \\ 
(dBm) & & & & \\ \hline
Avg. Power & 0.0\% & +70.6\% & +181.6\% & +158.2\% \\ 
Gain & & & & \\ \hline
Premature & 0.0\% & 41.0\% & 0.0\% & \textbf{3.5\%} \\ 
Switch Rate & & & & \\ \hline
Avg. Handover & 0 & 56 & 47 & 39 \\ 
Frequency & & & & \\ \hline
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% Ablation Study Table %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}
\caption{Enwar 3.0 Edge-Case and Ablation Study}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Scenario} & \textbf{\begin{tabular}[c]{@{}c@{}}Available\\ Modalities\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Beam\\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Blockage\\ F1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enwar 3.0 \\Judgement\\\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Final Action\\ \end{tabular}} \\ \hline

\begin{tabular}[c]{@{}c@{}}Clear weather, \\ ideal scenario\end{tabular} & All & 88.5\% & 98.4\% & \begin{tabular}[c]{@{}c@{}}All sensors functional; \\ select best model\end{tabular} & \begin{tabular}[c]{@{}c@{}}Use best model fusion \\ for both agents\end{tabular} \\ \hline

\begin{tabular}[c]{@{}c@{}}Heavy fog, \\ visual occlusion with \\average degradation 42.8\% \end{tabular} & \begin{tabular}[c]{@{}c@{}}GPS, LiDAR, radar \\ (camera degraded)\end{tabular} & 83.0\% & 93.7\% & \begin{tabular}[c]{@{}c@{}}Visual sensor degraded; \\ fallback to radar-based \\fusion models\end{tabular} & \begin{tabular}[c]{@{}c@{}}Use radar model \\for blockage, and \\GPS-radar-LiDAR \\fusion for beam\end{tabular} \\ \hline

\begin{tabular}[c]{@{}c@{}}Bright sun glare with \\average degradation 31.0\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}GPS, LiDAR,\\ radar\\ (camera occluded)\end{tabular} & 83.0\% & 93.7\% & \begin{tabular}[c]{@{}c@{}}Visual sensor degraded; \\ fallback to radar-based \\fusion models\end{tabular} & \begin{tabular}[c]{@{}c@{}}Use radar model \\for blockage, and \\GPS-radar-LiDAR \\fusion for beam\end{tabular} \\ \hline

\begin{tabular}[c]{@{}c@{}}Nighttime,\\ low visibility with \\average degradation 55.0\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}GPS, LiDAR,\\ radar\\ (camera degraded)\end{tabular} & 83.0\% & 93.7\% & \begin{tabular}[c]{@{}c@{}}Visual sensor degraded; \\ fallback to radar-based \\fusion models\end{tabular} & \begin{tabular}[c]{@{}c@{}}Use radar model \\for blockage, and \\GPS-radar-LiDAR \\fusion for beam\end{tabular} \\ \hline

\begin{tabular}[c]{@{}c@{}}GPS jamming with \\average degradation 37.2\% \end{tabular} & \begin{tabular}[c]{@{}c@{}}Camera, LiDAR,\\ radar\end{tabular}& 88.3\% & 98.4\% & \begin{tabular}[c]{@{}c@{}}GPS signal unreliable; use \\ camera-LiDAR-radar \\models\end{tabular} & \begin{tabular}[c]{@{}c@{}}Use camera-radar\\ for blockage, and\\ camera-radar-LiDAR\\ for beam\end{tabular} \\ \hline

\begin{tabular}[c]{@{}c@{}}LiDAR sensor \\ non-functional with \\average degradation 59.4\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Camera, GPS,\\ radar \end{tabular} & 84.9\% & 98.4\% & \begin{tabular}[c]{@{}c@{}}LiDAR fusion degraded;\\ fallback to radar-based\\ models\end{tabular} & \begin{tabular}[c]{@{}c@{}}Use to camera-radar\\ fusion for both agents\end{tabular}\\ \hline

\begin{tabular}[c]{@{}c@{}}Radar noisy \\ in rain with \\average degradation 39.9\%\end{tabular}& \begin{tabular}[c]{@{}c@{}}Camera, GPS, LiDAR \\ (radar noisy)\end{tabular} & 85.6\% & 98.1\% & \begin{tabular}[c]{@{}c@{}}Radar noise detected; \\ rely on camera-LiDAR\end{tabular} & \begin{tabular}[c]{@{}c@{}} Use camera-LiDAR\\ fusion for beam,\\ and camera model\\ for blockage\end{tabular} \\ \hline


\begin{tabular}[c]{@{}c@{}}Blockage longer than \\$t+5$ time steps confirmed,\\ BS2 RSSI higher\end{tabular} & All & 88.5\% & 98.4\% & \begin{tabular}[c]{@{}c@{}}Blockage confirmed,\\ BS2 power difference \\exceeds threshold\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trigger handover to \\BS2; use best \\fusion models \end{tabular}\\ \hline

\begin{tabular}[c]{@{}c@{}}LiDAR and radar\\ non-functional with \\average degradation 63.7\%\end{tabular} & Camera, GPS & 83.7\% & 94.4\% & \begin{tabular}[c]{@{}c@{}}LiDAR and radar degraded; \\ use camera-gps fusion models \end{tabular} & \begin{tabular}[c]{@{}c@{}}Use camera model\\ for blockage,\\ camera-GPS for\\ beam\end{tabular} \\ \hline
\end{tabular}
\label{tab: ablation_study_enwar3}
\end{table*}
